Mito-nuclear selection induces a trade-off between species ecological dominance and evolutionary lifespan

Mitochondrial and nuclear genomes must be co-adapted to ensure proper cellular respiration and energy production. Mito-nuclear incompatibility reduces individual fitness and induces hybrid infertility, suggesting a possible role in reproductive barriers and speciation. Here we develop a birth-death model for evolution in spatially extended populations under selection for mito-nuclear co-adaptation. Mating is constrained by physical and genetic proximity, and offspring inherit nuclear genomes from both parents, with recombination. The model predicts macroscopic patterns including a community's long-term species diversity, its species abundance distribution, speciation and extinction rates, as well as intra- and inter-specific genetic variation. We explore how these long-term outcomes depend upon the microscopic parameters of reproduction: individual fitness governed by mito-nuclear compatibility, constraints on mating compatibility, and ecological carrying capacity. We find that strong selection for mito-nuclear compatibility reduces the equilibrium number of species after a radiation, increases the species' abundances, while simultaneously increasing both speciation and extinction rates. The negative correlation between species diversity and diversification rates in our model agrees with the broad empirical pattern of lower species diversity and higher speciation/extinction rates in temperate regions, compared to the tropics. We therefore suggest that these empirical patterns may be caused in part by latitudinal variation in metabolic demands, and corresponding variation in selection on mito-nuclear function.

==> file.tex <==



==> file1.tex <==



==> preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{lmodern}
\usepackage{upgreek}
\usepackage{textcomp}
\usepackage{amsmath,amsfonts,amssymb,latexsym,amsthm,mathrsfs}
% \usepackage[mathscr]{euscript}
\usepackage[english]{babel} 
\usepackage{indentfirst,setspace,fancyhdr}
\usepackage[outercaption]{sidecap}
\usepackage[footnotesize]{caption}
\usepackage[margin=3cm]{geometry}
\usepackage[pdftex]{graphicx}
% \usepackage{epstopdf}
\usepackage{color,xcolor}
%\usepackage{uarial}
%\renewcommand{\familydefault}{\sfdefault}
%\usepackage{blindtext}
\usepackage[none]{hyphenat}
\usepackage[toc,page]{appendix}
%\usepackage{multicol}
\usepackage{colortbl}
%\usepackage{braket}
\usepackage{gensymb}
\usepackage{multirow}
\usepackage{array}
\usepackage{pstricks}
% \usepackage{import}
\usepackage{wrapfig}
% \usepackage{fancyref}
\usepackage{pdfpages}
\usepackage{mathtools}
\usepackage{booktabs} % Better table styles
\usepackage{cite}
%\usepackage{verbatim}                
%\usepackage{subfig}
% \usepackage{natbib}
% \setlength{\bibsep}{0.0pt}
\usepackage{quoting}
\usepackage{longtable}
\usepackage{cancel}
%\usepackage[usestackEOL]{stackengine}
\usepackage{makecell}
\usepackage{tikz,stackengine}
\usetikzlibrary{matrix,calc}
\usepackage{blkarray}
\usetikzlibrary{decorations.pathreplacing}
\renewcommand{\cellalign}{tl}
\usepackage{tabularx}
\usepackage{authblk}

\usepackage{setspace}\doublespacing


\usepackage{soul}
\usepackage[normalem]{ulem}

\usepackage{abstract}
\addto{\captionsenglish}{\renewcommand{\abstractname}{}}
\renewcommand{\absnamepos}{empty}

\newcommand*{\temp}{\multicolumn{1}{c|}{0}}
\newcommand{\diagentry}[1]{\mathmakebox[1.8em]{#1}}
\newcommand{\xddots}{%
	\raise 4pt \hbox {.}
	\mkern 6mu
	\raise 1pt \hbox {.}
	\mkern 6mu
	\raise -2pt \hbox {.}
}
\tolerance=1
\emergencystretch=\maxdimen
\hyphenpenalty=10000
\hbadness=10000

\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.10] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\graphicspath{{Figures/}} 
\newcolumntype{g}{>{\columncolor{light-gray}}c}

\usepackage{sectsty}
\allsectionsfont{\sffamily}

\usepackage[labelformat=empty, position=top]{subcaption}
% \usepackage[export]{adjustbox}

% Caption configuration
\setlength{\captionmargin}{20pt} % sets an extra marging of 20pt for the caption
\definecolor{Gray}{rgb}{0.5,0.5,0.5}
\definecolor{darkblue}{rgb}{0.12,0.15,0.49}
\definecolor{light-gray}{gray}{0.85}
\definecolor{mygreen}{rgb}{0, 0.5, 0}
%\usepackage[pdftex,linktocpage]{hyperref}
\geometry{a4paper,top=2.5cm,left=2.5cm,right=2.5cm,bottom=2.5cm} % Set margins
\setlength\parindent{1cm} 

\makeatletter
\renewcommand\@biblabel[1]{#1.} 
\makeatother
\allowdisplaybreaks

\usepackage[backgroundcolor=yellow!30,textsize=footnotesize]{todonotes}

\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
\myexternaldocument{supplementary}
